Measuring Moral Dimensions in Social Media with Mformer

The ever-growing textual records of contemporary social issues, often discussed online with moral rhetoric, present both an opportunity and a challenge for studying how moral concerns are debated in real life. Moral foundations theory is a taxonomy of intuitions widely used in data-driven analyses of online content, but current computational tools to detect moral foundations suffer from the incompleteness and fragility of their lexicons and from poor generalization across data domains. In this paper, we fine-tune a large language model to measure moral foundations in text based on datasets covering news media and long- and short-form online discussions. The resulting model, called Mformer, outperforms existing approaches on the same domains by 4--12% in AUC and further generalizes well to four commonly used moral text datasets, improving by up to 17% in AUC. We present case studies using Mformer to analyze everyday moral dilemmas on Reddit and controversies on Twitter, showing that moral foundations can meaningfully describe people's stance on social issues and such variations are topic-dependent. Pre-trained model and datasets are released publicly. We posit that Mformer will help the research community quantify moral dimensions for a range of tasks and data domains, and eventually contribute to the understanding of moral situations faced by humans and machines.

==> sections/mfd_limits.tex <==
\section{Moral Foundations Via Word Count}
\label{sec:wordcount_limits}

%\begin{itemize}
%	\item All MFD lexicons have limited vocabulary. This reveals a trade-off between having few words that are strong indicators but achieving low recall and having too many words with higher coverage but achieving higher false positive rates.
%	\item This also favors longer sequences (higher hit rate).
%	\item The association of words with moral foundations is subjective and can reveal bias. Example: father and mother in family topics.
%	\item The handling of word inflections is unclear.
%	\item The encoding of virtue or vice for each word...
%\end{itemize}

Word count methods based on lexicons remain the most popular for automatically detecting moral foundations in text. Here we detail how they work and several of their limitations when applied to text corpora.

\header{Scoring via lexicon} Each lexicon, called moral foundations dictionary (MFD), contains a list of words and the foundations they represent. For example, the word ``deceive'' can be mapped to the foundation \foundation{loyalty}. A document to be scored is first tokenized; then, for each token that is also in the MFD, the count for foundation the token is mapped to is incremented. For instance, if the token is ``deceive,'' then the count for \foundation{loyalty} is increased by one. 

\header{Available lexicons} We note three versions of the MFD that have been used extensively in the literature. The first MFD, released as a dictionary to be used in LIWC-like programs, contains nearly 600 words \citep{grahamMoralFoundationsDictionary2012}. Later, a new version with over 2K words called MFD 2.0 \citep{frimerMoralFoundationsDictionary2019c} was released in which the creators extended their expert-crafted word lists by querying a word embedding \cite{mikolovDistributedRepresentationsWords2013} for similar terms. Another recent variant, called the extended MFD (eMFD, 3.2K words) \citep{hoppExtendedMoralFoundations2021}, contains one-to-many mappings associated with moral foundation weights, between 0 and 1, for each word. We list some example words of these MFDs in \Cref{tab:mfd_example_words} in the appendix and show some overlap between them in \Cref{fig:mfds_aita_wordcount}.

\header{Limitations} Word count methods are easy to implement, involve no model training and are interpretable through showing what words directly signify a foundation. We find that, however, such scoring methods have several important limitations that can affect downstream measurements and how they are subsequently interpreted.

% 1. Lexicon sizes and their words:
% - Supposedly all words are morally relevant regarding the foundations they map to
% - Their overlap is very small
First, these lexicons have a fixed and limited vocabulary. See \Cref{fig:mfds_aita_wordcount} (left) above for some example words and a visualization. Most of the words in these lexicons are supposedly morally relevant, but their overlap is very small. For instance, the 281 words common to both MFD and MFD 2.0 only account for 47.5\% of MFD and 13.8\% of MFD 2.0. This percentage is even smaller when the eMFD is considered. When scoring a document, only counting words in one lexicon risks missing out valid candidate words in others. 

% This represents a trade-off between having few words that are strong indicators but achieving low recall and having too many words with higher coverage but achieving higher false positive rates, and how to balance this trade-off is unclear. 

% 2. Unclear how to handle word variants and derivations
% - The set of all inflections of each word is incomplete. This means that one needs to trace every word to its lexeme and the process is unclear.
% - How to handle morphological derivations, especially with respect to disambiguating parts of speech. -> Refer to Rezapour et al. for their version of the MFD including POS 
Second, when using the MFDs, it is unclear how word variations should be handled. For example, the MFD 2.0 explicitly contains the verb ``desecrate'' and its inflectional forms ``desecrates,'' ``desecrated'' and ``desecrating.'' However, this is not the case for the verb ``deify,'' which is in the lexicon, while ``deified'' is not. A direct, but possibly inexhaustive, way to address this is to lemmatize all tokens in a document before performing lexicon lookup. Another related issue is how to disambiguate the parts of speech of some words in these dictionaries. For example, given the word ``bully'' in the MFD 2.0, should it be counted when it is verb, noun or even adjective (which, in this case, means ``excellent'')? Some prior work has been dedicated to this disambiguation, most notably the ``extended MFD'' built on top of the MFD by \citet{rezapourEnhancingMeasurementSocial2019}. 

% 3. Favor longer texts
Third, the heuristic nature of word count suggests that longer documents tend to result in more dictionary matchings, which may favor longer sequences of text. To provide evidence for this, we score a sample of 6,800 Reddit posts and assess the relationship between a post's length and the number of words in that post which are found in each lexicon. The results, presented in \Cref{fig:mfd_word_count_vs_length_correlation} in the appendix, show that how many words in a post are found in a lexicon strongly relates to how long that post is. This holds true for all three versions: MFD, MFD 2.0 and eMFD. In \Cref{appn:mfd_limits}, we also show an example post that is predicted to underscore the foundation \foundation{authority} simply because it contains only one word which is mapped to this foundation. Predictions like this are arguably very unreliable and highlight the downside of word count on texts of different lengths.

% 4. Encode the bias of those who created the dictionaries
Finally, the association of words with moral foundations by ``experts'' reveals personal subjectivity and bias. In the same analysis using Reddit posts, we discover some problematic associations. \Cref{fig:mfds_aita_wordcount} (right) presents the most frequently matched words that are related to two foundations: \foundation{authority} and \foundation{care}. Using the MFD 2.0, some associations such as ``father'' with \foundation{authority} and ``mother'' with \foundation{care} appear to reflect the bias of the lexicon creators when assigning moral intuitions to very general familial roles.

Overall, we believe that detecting moral foundations by counting words in some fixed lexicon is an oversimplistic approach that may lead to very coarse predictions. Although some workarounds, such as augmenting the MFDs with part-of-speech tags, exist, they do not fully address the heuristic nature of these methods. We hence advocate for more sophisticated predictors that are grounded in machine learning. In the following sections, we describe our approach, called \ourmodel, based on fine-tuning a large language model using high-quality, public datasets. 
% In \Cref{sec:evaluation} we also present an extensive evaluation of MFormer's performance in comparison with existing methods, including word count.

% To illustrate these two points, we take 6,800 Reddit posts of the topic \topic{family} on \texttt{r/AmItheAsshole} \citep{nguyenMappingTopics1002022b}, containing over 2.9M tokens, and score them using the three lexicons. The result shows that many posts are considered to contain a foundation simply because they have only one word in the dictionary maps to that foundation. See \Cref{appn:mfd_limits} for some examples. As we show in \Cref{fig:mfds_aita_wordcount}, right, some associations such as ``father'' $\rightarrow$ \foundation{authority} and ``mother'' $\rightarrow$ \foundation{care} appear to reflect the bias of the creators of the MFD 2.0 when assigning moral intuitions to general familial roles.

% Alasdair's: maybe discuss the limitations of embedding similarity + logistic regression

==> sections/mfd_review.tex <==
\section{Related Work}
\label{sec:related_work}

Our work builds upon the literature on identifying key moral dimensions, detecting them in text, and measuring a variety of properties pertaining to morality within large corpora.

\subsection{Moral Foundations Theory}
\label{sec:related_work:MFT}

The moral foundations theory, developed in moral psychology, proposes a taxonomy over what are called ``moral intuitions'' \citep{haidtIntuitiveEthicsHow2004a,haidtRighteousMindWhy2012}. In an attempt to explain the similarities and differences in moral judgment, Haidt and colleagues discovered key categories of intuitions behind people's moral judgments. These so-called ``moral foundations'' underlie five notions: \foundation{authority/subversion}, relating to traits such as deference to higher authorities to maintain group cohesion; \foundation{care/harm}, upholding the virtues of nurturing and protection; \foundation{fairness/cheating}, involving equal treatment and reward; \foundation{loyalty/subversion}, relating to prioritizing one's group and alliances; and \foundation{sanctity/degradation}, including intuitions about maintaining the sacredness of the body and avoiding moral contamination. Anthropological evidence suggests that these foundations are universal and developed through evolution, although which traits constitute a virtue and which constitute a vice vary across cultures \citep{grahamMoralFoundationsTheory2013a}.

Most studies using the MFT have focused on characterizing political ideology, especially in the U.S. context. For example, pertaining to the foundations \foundation{care} and \foundation{fairness}, liberals often support the commitment to justice and actions that uphold equality and those that avoid or relieve suffering. Conservatives, on the other hand, tend to value all five foundations somewhat equally, additionally upholding virtues such as loyalty to one's country and respecting authority and order \citep{grahamLiberalsConservativesRely2009a,mcadamsFamilyMetaphorsMoral2008,haidtWhenMoralityOpposes2007,vanleeuwenPerceptionsSocialDangers2009}. The theory has also been used to characterize the differences in moral sentiment surrounding socially significant topics such as stem cell research \citep{cliffordHowWordsWork2013}, vaccine hesitancy \citep{aminAssociationMoralValues2017}, euthanasia, abortion, animal cloning and same-sex marriage \citep{kolevaTracingThreadsHow2012}.

% It is in this capacity that the theory has been used to study human moral beliefs in different, perhaps less morally loaded, domains.

\subsection{Automatically Detecting Moral Foundations}
\label{sec:related_work:MF_detection}

% Using moral foundations as features for documents has been shown useful in answering research questions in several domains, as described in \Cref{sec:intro}. As a result, there is a multitude of methods to detect, or score, MFs in text, from word counts based on hand-crafted lexicons to statistical models trained from annotated data. In this subsection, we review existing methods for scoring MFs in the literature. 

A common theme in most large-scale studies of the MFT is how to detect moral foundations automatically. While the gold standard in moral foundation labeling is human annotation, it becomes too costly to scale that effort, which requires extensive training and evaluation, to the size of these text collections \cite{hooverMoralFoundationsTwitter2020a,tragerMoralFoundationsReddit2022}. Here, we categorize the automatic scoring of moral foundations into word count, embedding similarity and supervised classification methods.

\emph{Word count methods} rely on a human-crafted lexicon, which is a mapping from word to foundation. When scoring a document, each token contained in the lexicon counts as one occurrence of the foundation that the token maps to. These methods bear resemblance to LIWC \citep{tausczikPsychologicalMeaningWords2010}, a popular computer program that scores many psychological and emotional features in text based on an expert-validated lexicon. In \Cref{sec:wordcount_limits} below, we review these methods in detail while highlighting their limitations.

% Similar to LIWC, lexicons used to detect moral foundations, typically called moral foundations dictionaries (MFDs), are constructed by humans. The first MFD, released as a dictionary to be used in LIWC-like programs \citep{grahamMoralFoundationsDictionary2012}, contains nearly 600 words. Later, a new version with over 2K words called MFD 2.0 \citep{frimerMoralFoundationsDictionary2019c} was released in which the creators extended their expert-crafted word lists by querying a word embedding \cite{mikolovDistributedRepresentationsWords2013} for similar terms. Another recent variant, called the extended MFD (eMFD, 3.2K words) \citep{hoppExtendedMoralFoundations2021}, contains one-to-many mappings associated with moral foundation weights, between 0 and 1, for each word. We list some example words of these MFDs in \Cref{tab:mfd_example_words} in the appendix and show some overlap between them in \Cref{fig:mfds_aita_wordcount}.

\emph{Embedding similarity methods} make use word embeddings like word2vec \cite{mikolovDistributedRepresentationsWords2013}. In this case, one also starts with a lexicon of word-to-foundation mappings. Each word is then embedded to a high-dimensional dense vector and every foundation is taken as the average of all word vectors describing it. To score a document, one first performs tokenization and maps all of its tokens to their vector embeddings. The document is then the average of all embeddings of its tokens. The relevance between a document and a foundation is defined as the cosine similarity between their vector representations. 
% The moral foundation frame bias and intensity in \citet{mokhberianMoralFramingIdeological2020b} used this method to define a frame for each foundation.

% Unsupervised aim to construct representations for moral foundations from the ground up, based on data annotated by many human annotators. The extended MFD (eMFD) \citep{hoppExtendedMoralFoundations2021} is one such example. The authors pulled around 1,000 news article from the GDELT dataset \cite{leetaruGDELTGlobalData2013a} and employed over 800 annotators to highlight the sections of each article that are about each foundation. Afterward, the foundation score for each word is defined as the frequency with which the word appears in a highlighted with this foundation. The result is a collection of over 3,000 words, each with five scores corresponding to the five foundations. This can be seen as a soft count of moral foundations for each word, compared to MFD and MFD 2.0; a document is also tokenized and the count for each foundation is replaced by the word scores.

\emph{Supervised classification methods} treat the detection of moral foundations as a text classification task. For example, \citet{hooverMoralFoundationsTwitter2020a} annotated a dataset of tweets and used it to train support vector machines to classify moral foundations. Similarly, using annotated social media data, \citet{tragerMoralFoundationsReddit2022} and \citet{liscioCrossDomainClassificationMoral2022} fine-tuned BERT \cite{devlinBERTPretrainingDeep2019}, a large language model, for the same task and reported the best known performance. In this paper, we also aim to build moral foundation classifiers learned from a number of high-quality annotated datasets.
% We describe the data sources in \Cref{sec:dataset} and the training process in \Cref{sec:classifiers}. We then compare existing methods with ours in \Cref{sec:evaluation}.

\subsection{MFT-Based Analyses of Text}
\label{sec:related_work:MFT_studies}

Adopting the MFT to analyses of moral sentiment has been the focus of a growing body of work in social psychology and digital humanities, most of which also examined political or ideological leaning \citep{gartenMoralityLinesDetecting2016,gartenDictionariesDistributionsCombining2018,johnsonClassificationMoralFoundations2018,xieTextbasedInferenceMoral2019,mokhberianMoralFramingIdeological2020b,hoppExtendedMoralFoundations2021,royIdentifyingMoralityFrames2021,rezapourIncorporatingMeasurementMoral2021}. For example, \citet{mokhberianMoralFramingIdeological2020b} studied the relationship between story framing and political leaning of several news sources. After using embedding similarity to score moral foundations, a statistical analysis found that on topics such as immigration and elections, conservative-leaning sources tend to underscore virtues of \foundation{sanctity} such as austerity and sacredness, while liberal-leaning sources emphasize the condemnation of vices like dirtiness and unholiness. In another work, \citet{rezapourIncorporatingMeasurementMoral2021} studied the relationship between moral foundations and stance (in favor, against or neutral) on several political topics discussed on Twitter. The authors used the MFD to detect foundations and subsequently found a significant relationship between, for example, the topic abortion and moral values surrounding foundations such as \foundation{care}, \foundation{loyalty} and \foundation{sanctity}.

Some prior work has made use of the MFT in other domains. For instance, \citet{hoppGraphLearningApproachDetecting2020} used the eMFD to analyze movie scripts and identified relevant foundations in movie scenes exhibiting moral conflicts. Using network-theoretic methods alongside moral foundations, the authors were able to construct communities of characters with specific shared moral characteristics. In argument mining, \citet{kobbeExploringMoralityArgumentation2020} proposed to use moral foundations, predicted using BERT, in the automatic assessment of arguments. The study found a significant correlation between moral sentiment (the presence of moral foundations) and audience approval of an argument. In another line of work, \citet{forbesSocialChemistry1012020} and \citet{ziemsMoralIntegrityCorpus2022} used the MFT to categorize collections of moral ``rules of thumb'' collected from large crowds and assessed large language models' moral predictions.

% In this paper, we also consider detecting moral foundations as a text classification task and experiment with many suitable approaches. Using data from several heterogeneous sources such as news articles, tweets and Reddit comments, we fine-tune a language model to score and classify moral foundations in text, achieving the best known performance on several benchmark datasets. We also provide an extensive evaluation and error analysis of all suitable methods described above, highlighting the merits and downsides of each. We describe the dataset in \Cref{sec:dataset} and the training process in \Cref{sec:classifiers}. The evaluation is presented in \Cref{sec:evaluation}. Finally, we demonstrate the utility of our MF classifiers in understanding and analyzing morally loaded content on Twitter and Reddit with two case studies in \Cref{sec:measurements}. 

% In addition to the news dataset used to create the eMFD by \citet{hoppExtendedMoralFoundations2021}, we identify two publicly released datasets on different domains. The MFs Twitter corpus \citep{hooverMoralFoundationsTwitter2020a} is a collection of 35K tweets across several topics such as Black Lives Matter, 2016 U.S. presidential election and hate speech. Each tweet is given MF labels by at least three trained annotators. Another recently released dataset is the MFs Reddit corpus \citep{tragerMoralFoundationsReddit2022}, which contains 16K Reddit comments across several subreddits such as r/antiwork and r/worldnews, along with MF annotations for each comment. The annotations are used as supervised signals for training MF classifiers. For example, \citet{hooverMoralFoundationsTwitter2020a} used the Twitter corpus to train SVMs and an LSTM model, and \citet{tragerMoralFoundationsReddit2022} also fine-tuned BERT \cite{devlinBERTPretrainingDeep2019} using the Reddit corpus to achieve a better performance.
